Parameterized Saga of First-Fit and Last-Fit Coloring

The classic greedy coloring (first-fit) algorithm considers the vertices of an input graph $G$ in a given order and assigns the first available color to each vertex $v$ in $G$. In the {\sc Grundy Coloring} problem, the task is to find an ordering of the vertices that will force the greedy algorithm to use as many colors as possible. In the {\sc Partial Grundy Coloring}, the task is also to color the graph using as many colors as possible. This time, however, we may select both the ordering in which the vertices are considered and which color to assign the vertex. The only constraint is that the color assigned to a vertex $v$ is a color previously used for another vertex if such a color is available. Whether {\sc Grundy Coloring} and {\sc Partial Grundy Coloring} admit fixed-parameter tractable (FPT) algorithms, algorithms with running time $f(k)n^{\OO(1)}$, where $k$ is the number of colors, was posed as an open problem by Zaker and by Effantin et al., respectively. Recently, Aboulker et al. (STACS 2020 and Algorithmica 2022) resolved the question for \Grundycol\ in the negative by showing that the problem is W[1]-hard. For {\sc Partial Grundy Coloring}, they obtain an FPT algorithm on graphs that do not contain $K_{i,j}$ as a subgraph (a.k.a. $K_{i,j}$-free graphs). Aboulker et al.~re-iterate the question of whether there exists an FPT algorithm for {\sc Partial Grundy Coloring} on general graphs and also asks whether {\sc Grundy Coloring} admits an FPT algorithm on $K_{i,j}$-free graphs. We give FPT algorithms for {\sc Partial Grundy Coloring} on general graphs and for {\sc Grundy Coloring} on $K_{i,j}$-free graphs, resolving both the questions in the affirmative. We believe that our new structural theorems for partial Grundy coloring and ``representative-family'' like sets for $K_{i,j}$-free graphs that we use in obtaining our results may have wider algorithmic applications.

==> Faster-Algo.tex <==
% !TEX root = Main.tex

We design a faster FPT algorithm for \pgc\ when the degeneracy of the input graph is bounded. Later, we explain how this algorithm and Theorem~\ref{thm:deg_reduction} can be used to design an FPT algorithm for the problem on general graphs. First, we design a randomized algorithm, and later we derandomize our algorithm using the “independence covering family”. We use the following result of Lokshtanov et al.~\cite{lokshtanov2020covering} in our algorithm.


%First, we design a randomized algorithm, and later we derandomize our algorithm using the ``independence covering family''. We use the following result of Lokshtanov et al.~\cite{lokshtanov2020covering} in our algorithm.
%\shortversion{ (for derandomization, see Section 3.2.1 of the full version)}

%\begin{definition}\label{def:grundy-witness}{\rm
%Let $G$ be a graph and $k$ be a positive integer.
%A sequence of pairwise disjoint independent sets $(Q_1,Q_2,\ldots,Q_k)$ of $G$ is a \emph{$k$-partial Grundy witness} if the following holds. For any $i \in [k]$, there is a vertex $v \in Q_i$ such that for all $j\in [i-1]$, $Q_j\cap N_G(v)\neq \emptyset$.
%Moreover, we say that a $k$-partial Grundy witness $(Q_1,Q_2,\ldots,Q_k)$ is \emph{properly colored} with respect to a coloring $\phi$ of $G$, if every vertex in $Q_i$ is colored with color $i$, for all $i\in [k]$. Here, we would like to mention that $\phi$ is not necessarily a proper coloring.
%}\end{definition}


%\begin{observation}\label{obs:k-witness-supset}
%Given a graph $G$ and an integer $k$, let $(Q_1,Q_2,\ldots,Q_k)$ be a $k$-partial Grundy witness.
%Suppose $Y_1,Y_2,\ldots,Y_k$ are pairwise disjoint independent sets in $G$ with the property that $Q_i\subseteq Y_i$ for all $i\in [k]$. Then, $(Y_1,Y_2,\ldots,Y_k)$ is also a $k$-partial Grundy witness of $G$.
%\end{observation}
%
%
%
%\begin{observation}\label{obs:k-witness}
%Given a graph $G$ and an integer $k$, let $(Q_1,Q_2,\ldots,Q_k)$ be a $k$-partial Grundy witness. Then, there exists a $k$-partial Grundy witness $(X_1,X_2,\ldots,X_k)$ such that for each $i\in [k]$, $X_i\subseteq Q_i$ and $|X_i|\leq k-i+1$.
%\end{observation}
%
%
%\begin{proof}
%For each $i\in [k]$, arbitrarily choose a vertex $u_i \in Q_i$ such that $N_G(u_i)\cap Q_j \neq \emptyset$ for all $j\in [i-1]$. We mark $u_i$ and one vertex from $N_G(u_i)\cap Q_j$ for all $j\in [i-1]$. Let $M$ be the set of all marked vertices. Then, $X_i=M\cap Q_i$ and $(X_1,X_2,\ldots,X_k)$ is the required $k$-partial Grundy witness.
%\end{proof}

\begin{proposition}[Lemma 1.1.~\cite{lokshtanov2020covering}] \label{lem:indcover}
There is a linear-time randomized algorithm that, given a $d$-degenerate graph $G$ and an integer $k$, outputs an independent set $Y$ such that for any independent set $X$ in $G$ with $|X|\leq k$, the probability that $X\subseteq Y$ is at least $\left({k(d+1) \choose k} \cdot k(d+1)\right)^{-1}$.
\end{proposition}

Using the above result, we next design a polynomial time randomized algorithm for the problem, where the success probability will not be that good; we will later make independent runs of this procedure to obtain the desired success probability.

\begin{lemma}\label{lem:random-degenerate}
There exists a polynomial-time randomized algorithm that, given an instance $(G,k)$ of \pgc, where $G$ is a $d$-degenerate graph, $k\in \mathbb{N}$, and does one of the following: i) outputs \no, or ii) outputs a $k$-partial Grundy witness, with the following guarantee. If $(G,k)$ is yes-instance, then the algorithm outputs a $k$-partial Grundy witness of $G$ with probability at least $(kd+k)^{-\probdpow}$. Moreover, if $(G,k)$ is no-instance, then the algorithm outputs {\sf No}. %\todo{The statement (ii) is not clear. Should we add "a partial Grundy witness $(G',k)$ with the following..." and replace $(G,k)$ with $(G',k)$?}
\end{lemma}

\begin{proof}
Let $(G,k)$ be the input instance of \pgc, where $G$ is a $d$-degenerate graph.
%We give a polynomial time randomized algorithm that returns a solution with probability at least $\left({k(d+1) \choose k} \cdot k^{k+1}(d+1)\right)^{-k}$ if $(G,k)$ is a yes-instance.
Our algorithm has the following steps:
\begin{enumerate}
\item Color all the vertices in $V(G)$ uniformly and independently at random with colors from the set $[k]$. Let the obtained coloring be $\phi : V(G)\rightarrow [k]$ and $Z_i=\phi^{-1}(i)$ for all $i\in [k]$.
%$Z_1,Z_2,\ldots,Z_k$ be the color classes.

\item For each $i\in [k]$, we run the algorithm of~\Cref{lem:indcover} for $(G[Z_i], k)$, and obtain an independent set $Y_i$.
% such that any independent subset of $Z_i$ with size at most $k$ is contained in $Y_i$.

\item If $(Y_1,Y_2,\ldots,Y_k)$ is a $k$-partial Grundy witness, then output $(Y_1,Y_2,\ldots,Y_k)$. Otherwise, output {\sf No}.
\end{enumerate}
Observe that the first and last steps can be performed in polynomial time. For the second step, we call the algorithm of~\Cref{lem:indcover} $k$ times, which runs in time linear in $n$. Hence, our algorithm runs in polynomial time.

Next, we prove the correctness of the algorithm. Suppose $(G,k)$ is a no-instance of \pgc. Then, our algorithm will output {\sf No}. Consider the case when $(G,k)$ is yes-instance. Then, there
is a $k$-partial Grundy witness $(X_1,X_2,\ldots,X_k)$ of $G$ such that $|X_i|\leq k-i+1$, for all $i\in [k]$ by Observation \ref{obs:k-witness}. 
We say that $(X_1,X_2,\ldots,X_k)$ is {\em valid} with respect to  a the random coloring $\phi$,  if $X_i\subseteq \phi^{-1}(i)$ for all $i\in [k]$.  Now, the probability that the $k$-partial Grundy witness $(X_1,X_2,\ldots,X_k)$ is valid  with respect to $\phi$ is at least ${k^{-k^2}}$.  
%by~\Cref{prop:color-coding}. In the second step, 

Next, 
we run the randomized algorithm of~\Cref{lem:indcover} that returns an independent set $Y_i\subseteq Z_i$ such that $\Pr[X_i\subseteq Y_i] \geq \left({k(d+1) \choose k} \cdot k(d+1)\right)^{-1}$, for each $i\in [k]$.
%any independent set of size at most $k$ is contained in $Y_i$ with probability at least $\left({k(d+1) \choose k} \cdot k(d+1)\right)^{-1}$. For simplicity, let $R=\left({k(d+1) \choose k} \cdot k(d+1)\right)^{-1}$.
By Observation~\ref{obs:k-witness-supset}, $(Y_1,Y_2,\ldots,Y_k)$ is a $k$-partial Grundy witness of $G$, if $X_i\subseteq Y_i$ for all $i\in [k]$.
Thus, the probability that $(Y_1,Y_2,\ldots,Y_k)$ is a $k$-partial Grundy witness of $G$ is at least $k^{-k^2}\left({k(d+1) \choose k} \cdot k(d+1)\right)^{-k} \geq (kd+k)^{-\probdpow}$.
%This completes the proof of the lemma.
% then from Observation \ref{obs:k-witness} there exists a $k$-partial Grundy witness $(X_1,X_2,\ldots,X_k)$ such that $X_i\subseteq Q_i$ and $|X_i|\leq k-i+1$, for each $i\in [k]$.
%Therefore, the probability that $(Y_1,Y_2,\ldots,Y_k)$ is a $k$-partial Grundy witness is at least the probability of the event that each $X_i\subseteq Y_i$ and $(X_1,X_2,\ldots X_k)$ is properly colored with respect to $\phi$. That is,$\Pi_{i=1}^{k} (Pr[X_i\subseteq Y_i]\cdot Pr[X_i \mbox{ is $i$-colored with respect to }\phi])$
%$\geq \Pi_{i=1}^{k}(R\cdot\frac{1}{k^{|X_i|}})\ \geq R^k\cdot\frac{1}{k^{k^2}} $.
%Hence, our algorithm returns a $k$-partial Grundy witness with probability at least $\frac{R^k}{k^{k^2}}$, that is, $\left({k(d+1) \choose k} \cdot k^{k+1}(d+1)\right)^{-k}$.
\end{proof}
By $(kd+k)^{\probdpow} \log n$ independent runs of the algorithm in Lemma~\ref{lem:random-degenerate}, we get the following.

\begin{theorem}
\label{thm:degeneracy}
There is an algorithm that given an instance $(G,k)$ of \pgc, where $G$ is a $d$-degenerate graph, runs in time
$(kd+k)^{2k^2+k} n^{\OO(1)}$ and it either outputs {\sf No} or a partial Grundy coloring of $G$ using at least $k$ colors with the following guarantee.
If $(G,k)$ is yes-instance, then the algorithm outputs a partial Grundy coloring of $G$ with probability at least %$\left({k(d+1) \choose k} \cdot k^{k+1}(d+1)\right)^{-k}$.
$1-\frac{1}{n}$. If $(G,k)$ is a no-instance, then the algorithm outputs {\sf No}. %\todo{Last 2 lines are not clear to me.}
\end{theorem}

\longversion{
\subparagraph{Derandomization.}\label{subsubsec:deran-one}
Next, we explain how to derandomize the algorithm in
Lemma \ref{lem:random-degenerate}. Towards this, we need the following definition and a known result.

\begin{definition}[$k$-Independence Covering Family~\cite{lokshtanov2020covering}]{\rm
For a graph $G$ and $k\in {\mathbb N}$, a family of independent sets of $G$ is a {\em $k$-{\icf}} for $(G,k)$, denoted by $ \ifam{G}{k}$, if for any independent set $X$ in $G$ of size at most $k$, there exists $Y \in \ifam{G}{k}$ such that $X \subseteq Y$.
}\end{definition}

\begin{proposition}[Lemma 3.2~\cite{lokshtanov2020covering}]
%[Deterministic Independence Covering Lemma]
\label{lemma:discl}
There is an algorithm that given a $d$-degenerate graph $G$ on $n$ vertices and $m$ edges, and $k\in {\mathbb N}$, in time bounded by $\OO(\binom{k(d+1)}{k} \cdot 2^{o(k(d+1))} \cdot (n+m)\log n)$, outputs a $k$-{\icf} for $(G,k)$ of size at most $\binom{k(d+1)}{k} \cdot 2^{o(k(d+1))} \cdot \log n$.%,where, $n=\vert V(G)\vert$ and $m=\vert E(G)\vert$.
\end{proposition}

Now, we are ready to derandomize the algorithm of Lemma \ref{lem:random-degenerate} and to get a deterministic algorithm for the \pgc~problem on $d$-degenerate graphs. To do that, we would derandomize the two random steps of the algorithm: Step 1 and Step 2.

Without loss of generality, we can assume that $V(G)=[n]$. For the first step, we can invoke~\Cref{obs:derandom} with $p= k^2$ and $q =k$, and compute a family of at most $k^{k^2} \cdot k^{\OO(\log k)}\cdot\log^2 n$ functions $\C{Q}$ from $[n]$ to $[k]$ in time bounded by $k^{k^2} \cdot k^{\OO(\log k)}\cdot n \log^2 n$ with the following guarantee. For any fixed small $k$-partial Grundy witness $(X_1,X_2, \cdots, X_k)$ in $G$ (if it exists), there is a function $\chi \in \C{Q}$ such that for each $i \in [k]$ and $v \in X_i$, we have $\chi(v) =i$; note that such a coloring is a good coloring. %Our algorithm, instead of working with a random coloring, can now iterate over the coloring functions in the set $\C{Q}$.

%we would like to replace the random choice of coloring $\phi$ of $V(G)$ into $k$ colors with an iteration over a set of coloring obtained from an $(n,k^2,k)$-universal set $\mathcal{U}$ of cardinality $k^{k^2}k^{\OO(\log k)}\cdot \log^2 n$. Let $v_1,\ldots,v_n$ be the vertices of $G$ in an arbitrary order. Then, for any vector $x\in \mathcal{U}$, we construct a coloring $\phi_x$ as follows.
%For each $i\in [n]$, $\phi_x(v_i)=x[i]$. Notice that if $(G,k)$ is a yes-intance, then there is a partial $k$-Grundy witness $(X_1,\ldots,X_k)$ of $G$ such that $\sum_{i\in [k]} |X_i| \leq k^2$. Then, by the definition of $(n,k^2,k)$-universal set $\mathcal{U}$, there is a vector $x\in \mathcal{U}$ such that $X_i\subseteq \phi_x^{-1}(i)$.

% from Proposition \ref{prop:universal-set} some pseudo-randomobject. To do that we construct an $(n,k^2,k)$-universal set $U(G,k)$ from Proposition \ref{prop:universal-set}, with cardinality
Now for each $\phi \in \C{Q}$, we do the following instead of Step 2. For each $i\in [k]$, let $Z_i=\phi^{-1}(i)$. Construct a $k$-{\icf}
$\mathcal{F}(G[Z_i],k)$ that covers all independent sets in $Z_i$ of size at most $k$, for each $i\in [k]$. Clearly, if $X_i \subseteq Z_i$, then there is an independent set in $\mathcal{F}(G[Z_i],k)$ that contains $X_i$, for $i \in [k]$. Thus, if
there is a tuple in $\mathcal{F}(G[Z_1],k) \times \mathcal{F}(G[Z_2],k) \times \ldots \times \mathcal{F}(G[Z_k],k) $ which is a $k$-partial Grundy witness, then we output it (See Observation~\ref{obs:k-witness-supset}). If for each $\phi \in \C{Q}$, we fail to find a $k$-partial Grundy witness, then we output {\sf No}.


%Therefore, we deterministically find the independent set $Y_i$ from the family $\mathcal{F}(G[Z_i],k)$, for each color class $Z_i$ corresponding to a fixed coloring $\phi$. From Lemma \ref{lemma:discl}, we construct such a $k$-independence covering family of size at most $\binom{k(d+1)}{k} \cdot 2^{o(k(d+1))} \cdot \log n$.
%
%As the last step of our deterministic algorithm, we check for each possible combination of independent sets $Y_1,Y_2,\ldots,Y_k$ such that for every set $Y_i\in \mathcal{F}(G[Z_i,k)$, for all $i\in [k]$, whether $(Y_1,Y_2,\ldots,Y_k)$ is a $k$-partial Grundy witness. Given any $k$-partial Grundy witness $(Y_1,Y_2,\ldots,Y_k)$, the algorithm returns a partial Grundy $k$-coloring where each set $Y_i$ is colored with color $i$, for $i\in [k]$. Otherwise, the algorithm returns that $(G,k)$ is NO-instance.
%
%For simiplicity, let us assume that $R=k^{k^2}k^{\OO(\log k)}\cdot \log^2 n$ and $S=\binom{k(d+1)}{k} \cdot 2^{o(k(d+1))} \cdot \log n$.

%\smallskip
%\noindent
%\textbf{Running time.}
The correctness of the above procedure follows from~\Cref{obs:derandom},~\Cref{lemma:discl}, and the proof of~\Cref{lem:random-degenerate}. Let $R=k^{k^2}k^{\OO(\log k)}\cdot \log^2 n$ and $S=\binom{k(d+1)}{k} \cdot 2^{o(k(d+1))} \cdot \log n$.
The time required to compute the family $\C{Q}$ is bounded by $\C{O}(R \cdot n)$, and the number of functions in $\C{Q}$ is at most $R$. %The time taken to construct an $(n,k^2,k)$-universal set is $\OO(R\cdot n)$.
For a fixed coloring $\phi$, the time taken to construct a $k$-\icf~ $\mathcal{F}(G[Z_i],k)$ is $\OO(S \cdot (n+m))$, for each $i\in [k]$. For a fixed $\phi\in \C{Q}$, the running time to execute Step 2 is
$ \OO(S\cdot (n+m))+ \left( \Pi_{i=1}^{k} |\mathcal{F}(G[Z_i],k)|\right)\cdot n^{\OO(1)}=S^k\cdot n^{\OO(1)}=(k+dk)^{\OO(k^2)} n^{\OO(1)}$, because $(\log n)^k$ is upper bounded by $\OO(2^{k\log k} n)$.\footnote{If $n \leq k^k$,  then $\log n \leq k\log k$ and $(\log n)^k\in \OO(2^{k\log k} n)$.  Otherwise,  $k \in \OO(\log n/\log \log n)$, and $(\log n)^k \in n^{\OO(1)}$ (see, for instance, Ex. 3.18 and its hint from~\cite{cygan2015parameterized}).} Therefore, the total running time is upper bounded by $(k+dk)^{\OO(k^2)} n^{\OO(1)}$. Thus, we get a proof of~\Cref{thm:degeneracydet}.
 
 }

%Recall that the number of possible colorings of $V(G)$ is the cardinality of the universal set $\mathcal{U}(G,k)$, that is, $R$, and the time complexity to construct such a universal set is $\OO(R\cdot n)$.

%$\OO(R\cdot n)+R\cdot \OO( S^2\cdot n^{\OO(1)})$, that is, $\OO(R\cdot S^2\cdot n^{\OO(1)})$. Hence, we design a deterministic algorithm with running time $\OO(k^{k^2}k^{\OO(\log k)}\cdot \log^2 n\cdot \left(\binom{k(d+1)}{k} \cdot 2^{o(k(d+1))} \cdot \log n\right)^2\cdot n^{\OO(1)})$, that is, $\OO^*(k^{k^2}k^{\OO(\log k)}\cdot \left(\binom{k(d+1)}{k} \right)^2\cdot 2^{o(k(d+1))})$.



==> additional-proofs.tex <==
\begin{observation}\label{obs:grundy-witness-closure}
Consider $k \in \mathbb{N}\setminus \{0\}$, a graph $G$ and a $k$-Grundy witness ${\sf wit}: V(T_k) \rightarrow V(G)$ for $G$. For each $q \in [k-1]$, ${\sf wit}|_{V(T_{q})}$ is a $q$-Grundy witness for $G$. 
\end{observation}
\begin{proof}
Let  ${\sf wit}: V(T_k) \rightarrow V(G)$ be a   $k$-Grundy witness for $G$. Then by Definition \ref{def:grundy-witness-uncol}, for each $q\in [k]$,  $\{{\sf wit}(t) \mid t \in V(T_k) \mbox{ and } \ell_k(t) = q\}$ is an independent set in $G$. It implies that for any $q\in[k-1]$ and $r\in [q]$,  $\{{\sf wit}(t) \mid t \in V(T_q) \mbox{ and } \ell_q(t) = r\}$ is an independent set in $G$ as $\ell_k(t)=\ell_r(t)$ by Definition \ref{def:grundy-tree-new}. Since $T_q$ is a subtree of tree $T_k$ for any $q\in [k-1]$, properties $2$ and $3$ of Definition \ref{def:grundy-witness-uncol} holds for each $t,t'\in V(T_q)$ and $(t,t')\in E(T_q)$. Hence, ${\sf wit}|_{V(T_{q})}$ is a $q$-Grundy witness for $G$ for each $q\in [k-1]$.
\end{proof}

\begin{observation}\label{obs:good-prob}
The coloring $\chi$ is nice with probability at least {\em blah}.
\end{observation}
\begin{proof}
The coloring $\chi$ is nice, if for each $q\in [k]$ and $v\in \what{V}_{{\sf wit},q}$, $\chi(v)=q$. Note that the size of $\what{V}_{{\sf wit},q}$ is same as the number of subtrees $T_q$ in $T_k$, that is, $2^{k-(q+1)}$, for any $q\in[k-1]$. Moreover, the size of $\what{V}_{{\sf wit},k}$ is $1$. Now, the probability that the coloring $\chi$ assigns the color $q$ to all the vertices in $\what{V}_{{\sf wit},q}$ ia at least $\frac{1}{k}^{|\what{V}_{{\sf wit},q}|}$.  Therefore, the probability that the coloring $\chi$ is nice,
\begin{equation*}

 & = \Pi_{q=1}^{k} \mbox {Pr[vertices of } \what{V}_{{\sf wit},q} \mbox{ are colored with color } q]\\
& \geq  \Pi_{q=1}^{k}  \frac{1}{k}^{|\what{V}_{{\sf wit},q}|}\\
& \geq  \Pi_{q=1}^{k-1}  (\frac{1}{k})^{2^{k-(q+1)}}\cdot \frac{1}{k} \geq (\frac{1}{k})^{2^{k^2}}.

\end{equation*}
\end{proof}


\begin{observation}\label{obs:transitive-vec-rep}
Consider $p \in \mathbb{N}$, a vector $\vec{q} = (q_1,q_2,\cdots, q_k)$, and (not necessarily disjoint) $p$-families $\C{F}_1$ and $\C{F}_2$. If $\C{F}'_1 \subseteq^{\vec{q}}_{grep} \C{F}_1$ and $\C{F}'_2 \subseteq^{\vec{q}}_{grep} \C{F}_2$, then $\C{F}'_1 \cup \C{F}'_2 \subseteq^{\vec{q}}_{grep} \C{F}_1 \cup \C{F}_2$. 
\end{observation}

\begin{proof}
Consider a set $B$ of size $\vec{q}$ such that there is some set $A\in \C{F}_1\cup \C{F}_2$ that fits $B$. If $A\in \C{F}_1$, then there exists some $A'\in \C{F}'_1$ that fits $B$ as $\C{F}'_1 \subseteq^{\vec{q}}_{grep} \C{F}_1$. If $A\in \C{F}_2$, then there exists some $A'\in \C{F}'_2$ that fits $B$ as $\C{F}'_2 \subseteq^{\vec{q}}_{grep} \C{F}_2$. Thus, there exists $A'\in \C{F}'_1\cup\C{F}'_2$ that fits $B$. Hence, $\C{F}'_1 \cup \C{F}'_2 \subseteq^{\vec{q}}_{grep} \C{F}_1 \cup \C{F}_2$.
\end{proof}


\begin{observation}\label{obs:transitive-vec-rep-one-vertex}
Consider $p \in \mathbb{N}$, a vector $\wvec{q} = (q_1,q_2,\cdots, q_k)$, a vertex $v \in V(G)$ and a $(p,v)$-family $\C{F}$. Let $\wvec{h}$ be the vector obtained from $\wvec{q}$ by increasing its $\chi(v)$th coordinate by $1$. If $\C{F}' \qrep{h} \C{F}-v$, then $\C{F}' + v \qrep{q} \C{F}$. 
\end{observation}

\begin{proof}
Consider a set $B$ of size $\vec{q}$ such that there is some set $A\in \C{F}$ that fits $B$. Since $\C{F}$ is a $(p,v)$-family, $v\in A$. Clearly, $A\setminus \{v\}\in \C{F}-v$ and $B\setminus \{v\}$ is of size $\vec{h}$. Now, there exists a set $A'\in \C{F}'$ that fits $B\setminus \{v\}$ as $\C{F}'\qrep{h} \C{F}-v$. It follows that $A'\cup\{v\} \in \C{F}'+v $ and $A'\cup\{v\} $ fits $B$. Hence, $\C{F}' + v \qrep{q} \C{F}$.
\end{proof}
